Flow From Motion: A Deep Learning Approach

Wearable devices have the potential to enhance sports performance, yet they are not fulfilling this promise. Our previous studies with 6 professional tennis coaches and 20 players indicate that this could be due the lack of psychological or mental state feedback, which the coaches claim to provide. Towards this end, we propose to detect the flow state, mental state of optimal performance, using wearables data to be later used in training. We performed a study with a professional tennis coach and two players. The coach provided labels about the players' flow state while each player had a wearable device on their racket holding wrist. We trained multiple models using the wearables data and the coach labels. Our deep neural network models achieved around 98% testing accuracy for a variety of conditions. This suggests that the flow state or what coaches recognize as flow, can be detected using wearables data in tennis which is a novel result. The implication for the HCI community is that having access to such information would allow for design of novel hardware and interaction paradigms that would be helpful in professional athlete training.

==> references.tex <==
\begin{thebibliography}
@article{Ioffe2015,
abstract = {Training Deep Neural Networks is complicated by the fact that the distribution of each layer's inputs changes during training, as the parameters of the previous layers change. This slows down the training by requiring lower learning rates and careful parameter initialization, and makes it notoriously hard to train models with saturating nonlinearities. We refer to this phenomenon as internal covariate shift, and address the problem by normalizing layer inputs. Our method draws its strength from making normalization a part of the model architecture and performing the normalization for each training mini-batch. Batch Normalization allows us to use much higher learning rates and be less careful about initialization. It also acts as a regularizer, in some cases eliminating the need for Dropout. Applied to a state-of-the-art image classification model, Batch Normalization achieves the same accuracy with 14 times fewer training steps, and beats the original model by a significant margin. Using an ensemble of batch-normalized networks, we improve upon the best published result on ImageNet classification: reaching 4.9{\%} top-5 validation error (and 4.8{\%} test error), exceeding the accuracy of human raters.},
archivePrefix = {arXiv},
arxivId = {1502.03167},
author = {Ioffe, Sergey and Szegedy, Christian},
eprint = {1502.03167},
month = {feb},
title = {{Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift}},
url = {http://arxiv.org/abs/1502.03167},
year = {2015}
}
@inproceedings{nair2010rectified,
author = {Nair, Vinod and Hinton, Geoffrey E},
booktitle = {Proceedings of the 27th international conference on machine learning (ICML-10)},
pages = {807--814},
title = {{Rectified linear units improve restricted boltzmann machines}},
year = {2010}
}
@article{lecun1998gradient,
author = {LeCun, Yann and Bottou, L{\'{e}}on and Bengio, Yoshua and Haffner, Patrick},
journal = {Proceedings of the IEEE},
number = {11},
pages = {2278--2324},
publisher = {IEEE},
title = {{Gradient-based learning applied to document recognition}},
volume = {86},
year = {1998}
}
@article{srivastava2014dropout,
author = {Srivastava, Nitish and Hinton, Geoffrey E and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
journal = {Journal of machine learning research},
number = {1},
pages = {1929--1958},
title = {{Dropout: a simple way to prevent neural networks from overfitting.}},
volume = {15},
year = {2014}
}
@inproceedings{chernbumroong2011activity,
author = {Chernbumroong, Saisakul and Atkins, Anthony S and Yu, Hongnian},
booktitle = {SKIMA},
organization = {IEEE},
title = {{Activity classification using a single wrist-worn accelerometer}},
year = {2011}
}
@article{um2016exercise,
author = {Um, Terry Taewoong and Babakeshizadeh, Vahid and Kulic, Dana},
journal = {arXiv preprint arXiv:1610.07031},
title = {{Exercise Motion Classification from Large-Scale Wearable Sensor Data Using Convolutional Neural Networks}},
year = {2016}
}
@inproceedings{connaghan2011multi,
author = {Connaghan, Damien and Kelly, Phillip and O'Connor, Noel E and Gaffney, Mark and Walsh, Michael and O'Mathuna, Cian},
booktitle = {Sensors},
organization = {IEEE},
pages = {1437--1440},
title = {{Multi-sensor classification of tennis strokes}},
year = {2011}
}
@misc{GPS,
booktitle = {Official U.S. government information about the Global Positioning System (GPS) and rekated topics},
title = {{GPS Accuracy}},
url = {https://www.gps.gov/systems/gps/performance/accuracy/},
year = {2017}
}
@inproceedings{havlucu2017understanding,
author = {Havlucu, Hayati and Bostan, Idil and Coskun, Aykut and {\"{O}}zcan, {\"{O}}guzhan},
booktitle = {Proc. CHI '17 Extended Abstracts},
organization = {ACM},
pages = {1678--1685},
title = {{Understanding the Lonesome Tennis Players: Insights for Future Wearables}},
year = {2017}
}
@book{kapp2012gamification,
author = {Kapp, Karl M},
publisher = {John Wiley {\&} Sons},
title = {{The gamification of learning and instruction: game-based methods and strategies for training and education}},
year = {2012}
}
@article{ledger2014inside,
author = {Ledger, Dan and McCaffrey, Daniel},
journal = {Endeavour Partners},
title = {{Inside wearables: How the science of human behavior change offers the secret to long-term engagement}},
volume = {200},
year = {2014}
}
@inproceedings{lazar2015we,
author = {Lazar, Amanda and Koehler, Christian and Tanenbaum, Joshua and Nguyen, David H},
booktitle = {Proceedings of the 2015 ACM International Joint Conference on Pervasive and Ubiquitous Computing},
organization = {ACM},
pages = {635--646},
title = {{Why we use and abandon smart devices}},
year = {2015}
}
@article{sweetser2005gameflow,
author = {Sweetser, Penelope and Wyeth, Peta},
journal = {Computers in Entertainment (CIE)},
number = {3},
pages = {3},
publisher = {ACM},
title = {{GameFlow: a model for evaluating player enjoyment in games}},
volume = {3},
year = {2005}
}
@book{jackson1999flow,
author = {Jackson, Susan A and Csikszentmihalyi, Mihaly},
publisher = {Human Kinetics},
title = {{Flow in sports}},
year = {1999}
}
@article{de2010psychophysiology,
author = {{De Manzano}, {\"{O}}rjan and Theorell, T{\"{o}}res and Harmat, L{\'{a}}szl{\'{o}} and Ull{\'{e}}n, Fredrik},
journal = {Emotion},
number = {3},
pages = {301},
publisher = {American Psychological Association},
title = {{The psychophysiology of flow during piano playing.}},
volume = {10},
year = {2010}
}
@book{gallwey2014inner,
author = {Gallwey, W Timothy},
publisher = {Pan Macmillan},
title = {{The inner game of tennis: The ultimate guide to the mental side of peak performance}},
year = {2014}
}
@inproceedings{maia2016study,
author = {Maia, Camila Loiola Brito and Furtado, Elizabeth S},
booktitle = {Proceedings of the 15th Brazilian Symposium on Human Factors in Computer Systems},
organization = {ACM},
pages = {7},
title = {{A study about psychophysiological measures in user experience monitoring and evaluation}},
year = {2016}
}
@article{Hochreiter1997,
author = {Hochreiter, Sepp and Schmidhuber, J{\"{u}}rgen},
doi = {10.1162/neco.1997.9.8.1735},
issn = {0899-7667},
journal = {Neural Computation},
month = {nov},
number = {8},
pages = {1735--1780},
title = {{Long Short-Term Memory}},
url = {http://www.mitpressjournals.org/doi/10.1162/neco.1997.9.8.1735},
volume = {9},
year = {1997}
}
@article{scikit-learn,
 title={Scikit-learn: Machine Learning in {P}ython},
 author={Pedregosa, F. and Varoquaux, G. and Gramfort, A. and Michel, V.
         and Thirion, B. and Grisel, O. and Blondel, M. and Prettenhofer, P.
         and Weiss, R. and Dubourg, V. and Vanderplas, J. and Passos, A. and
         Cournapeau, D. and Brucher, M. and Perrot, M. and Duchesnay, E.},
 journal={Journal of Machine Learning Research},
 volume={12},
 pages={2825--2830},
 year={2011}
}

@article{ledger2014inside,
  title={Inside wearables: How the science of human behavior change offers the secret to long-term engagement},
  author={Ledger, Dan and McCaffrey, Daniel},
  journal={Endeavour Partners},
  volume={200},
  number={93},
  pages={1},
  year={2014}
}
@inproceedings{Lazar:2015:WWU:2750858.2804288,
 author = {Lazar, Amanda and Koehler, Christian and Tanenbaum, Joshua and Nguyen, David H.},
 title = {Why We Use and Abandon Smart Devices},
 booktitle = {Proc. UbiComp '15},
 year = {2015},
 isbn = {978-1-4503-3574-4},
 location = {Osaka, Japan},
 pages = {635--646},
 numpages = {12},
 acmid = {2804288},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {personal informatics systems, self tracking, smart devices, wearable devices},
} 

@misc{csikszentmihalyi1990flow,
  title={Flow: The psychology of optimal performance},
  author={Csikszentmihalyi, Mihaly},
  year={1990},
  publisher={New York: Harper and Row}
}

@inproceedings{strasnick2017brushtouch,
  title={BrushTouch: Exploring an Alternative Tactile Method for Wearable Haptics},
  author={Strasnick, Evan and Cauchard, Jessica R and Landay, James A},
  booktitle={Proceedings of the 2017 CHI Conference on Human Factors in Computing Systems},
  pages={3120--3125},
  year={2017},
  organization={ACM}
}

@article{bian2016framework,
  title={A framework for physiological indicators of flow in VR games: construction and preliminary evaluation},
  author={Bian, Yulong and Yang, Chenglei and Gao, Fengqiang and Li, Huiyu and Zhou, Shisheng and Li, Hanchao and Sun, Xiaowen and Meng, Xiangxu},
  journal={Personal and Ubiquitous Computing},
  volume={20},
  number={5},
  pages={821--832},
  year={2016},
  publisher={Springer}
}

@inproceedings{nacke2008flow,
  title={Flow and immersion in first-person shooters: measuring the player's gameplay experience},
  author={Nacke, Lennart and Lindley, Craig A},
  booktitle={Proceedings of the 2008 Conference on Future Play: Research, Play, Share},
  pages={81--88},
  year={2008},
  organization={ACM}
}

@inproceedings{ahn2016pet,
  title={Pet Buddy: A wearable device for canine behavior recognition using a single IMU},
  author={Ahn, Juneyoung and Kwon, Jini and Nam, Hyejeong and Jang, Hyun-Kook and Kim, Jee-In},
  booktitle={Big Data and Smart Computing},
  pages={419--422},
  year={2016},
  organization={IEEE}
}

@inproceedings{spriggs2009temporal,
  title={Temporal segmentation and activity classification from first-person sensing},
  author={Spriggs, Ekaterina H and De La Torre, Fernando and Hebert, Martial},
  booktitle={Computer Vision and Pattern Recognition Workshops, 2009. CVPR Workshops 2009. IEEE Computer Society Conference On},
  pages={17--24},
  year={2009},
  organization={IEEE}
}
\end{thebibliography}
